Towards Robust and Automatic Hyper-Parameter Tunning

The task of hyper-parameter optimization (HPO) is burdened with heavy computational costs due to the intractability of optimizing both a model's weights and its hyper-parameters simultaneously. In this work, we introduce a new class of HPO method and explore how the low-rank factorization of the convolutional weights of intermediate layers of a convolutional neural network can be used to define an analytical response surface for optimizing hyper-parameters, using only training data. We quantify how this surface behaves as a surrogate to model performance and can be solved using a trust-region search algorithm, which we call autoHyper. The algorithm outperforms state-of-the-art such as Bayesian Optimization and generalizes across model, optimizer, and dataset selection. Our code can be found at \url{https://github.com/MathieuTuli/autoHyper}.

==> sections/related_works.tex <==
\subsection{Related Works}\label{sec_related_works}
% \subsection{Notation}
% For an integer $I \in \mathbb{Z}$, we denote the set of values from $1$ to $I$ as $[I] \leftarrow \{1, \hdots, I\}$. For some vector $a \in \mathbb{R}^b$, $a_i$ is the $i$th element along that vector. For some matrix $\boldsymbol{A} \in \mathbb{R}^{b\times c}$, $\boldsymbol{A}_i;\ i \in [b]$ is the $i$th vector across rows of $\boldsymbol{A}$ and element $\boldsymbol{A}_{i,j};\ i \in [b],\ j \in [c]$ is the $j$th element in the $i$th row-vector of $\boldsymbol{A}$.

% \subsection{Hyper-parameter Optimization}

% related works: year 2010 and before
% \cite{bengio2000gradient} - gradient based, non-deep learning

% related works: year 2011
% \cite{bergstra2011algorithms} - epexted improvement response surface

% related works: year 2012
% \cite{bergstra2012random} - random, defines surface response

% \cite{snoek2012practical} - bo technique

% related works: year 2013
% \cite{bergstra2013hyperopt} - lib for hpo

% \cite{bergstra2013making} - extesnsion of hpo for high number of dimensions (ask mahdi where to cat)

% \cite{eggensperger2013towards} - lib for hpo (also bo?) i added under bo

% \cite{karnin2013almost} - multi bandit (sha)
% related works: year 2014
% related works: year 2015
% \cite{feurer2015efficient} - bo

% \cite{maclaurin2015gradient}  - phsyica reversse hyperdynamics

% \cite{young2015optimizing} - genetic algorithm (pbt)

% \cite{feurer2015initializing} -  bo

% \cite{snoek2015scalable} - nn

% \cite{domhan2015speeding} - learning curve


% related works: year 2016
% \cite{luo2016review}  - review paper

% \cite{springenberg2016bayesian} - neural networks

% related works: year 2017
% \cite{li2017hyperband} - multi bandit

% \cite{jaderberg2017population} - pbt

% \cite{kotthoff2017auto} - lib

% \cite{klein2017fast} - bo

% \cite{diaz2017effective} - derivative free optimization boxz constrained

% related works: year 2018
% \cite{falkner2018bohb} - bo + multi bandit

% \cite{liaw2018tune} - lib

% \cite{li2018massively} - multi bandit

% related works: year 2019
% \cite{akiba2019optuna} - lib

% \cite{he2019automl} - review

% \cite{zhang2019deep} - orthanogal array

% related works: year 2020
% \cite{yu2020hyper}


%%%====== NEW FROM INTRO
We leave extensive analysis of the related works to established surveys \citep{luo2016review, he2019automl, yu2020hyper} but present a general overview here. Grid searching and manual tuning techniques that require extensive domain knowledge trial various configurations and retain the best. Random search \citep{bergstra2012random} was proven to be more efficient, particularly in high-dimensional cases, but these methods suffer from redundancy and high computational overhead. Bayesian Optimization (BO) \citep{snoek2012practical, eggensperger2013towards, feurer2015efficient, feurer2015initializing, klein2017fast} techniques attempt to characterize the distribution model of the random hyper-parameter configurations. They fail to properly define the response surface $\tau$ and resolve to estimating it by rationalizing a Gaussian Process (GP) over sampling points. The use of neural networks over GP \cite{snoek2015scalable, springenberg2016bayesian} to model the generalization performance was shown to have better computational performance. 

Multi-bandit -- also known as early-stopping - methods \citep{karnin2013almost, li2017hyperband, li2018massively} spawn various configurations with equal resource distributions, successively stopping poor performing configurations and reassigning resources dynamically. Population-based training (PBT) methods \citep{young2015optimizing, jaderberg2017population} follow an evolutionary approach by spawning various experimental configurations and adapting poor performing trials to warm restart with inherited learnable parameters and hyper-parameters. PBT methods are the most efficient methods thus far. In addition, other methods such as orthogonal array tuning \citep{zhang2019deep}, box-constrained derivative free optimization \citep{diaz2017effective}, reverse dynamics algorithm for SGD optimization \citep{maclaurin2015gradient}, and hybrid methods \citep{swersky2013multi, swersky2014freeze, domhan2015speeding, falkner2018bohb, kandasamy2016gaussian} exist but demonstrate no significant benefits over the previous techniques. 

Generally, each of these methods suffer from high computational overheads -- on the order of days to weeks to converge -- as well as additional internal hyper-parameters that heavily influence performance and generalization.

In recent years, many Python libraries have also been developed that include these optimization methods \citep{bergstra2013hyperopt, kotthoff2017auto, akiba2019optuna}. Cloud-based frameworks including Amazon Web Services and Google Visier exist as well.

%%%====== OLD STUFF
% Hyper-parameter optimization, and in particular initial learning rate selection, garners a lot of attention. To date, grid search, random search, and manual search techniques are most widely used to accomplish this task \citep{bergstra2012random}. In typical fashion, we aim to optimize (either minimize or maximize) some objective function $f(\Parameters;\HyperParameters)$ over a set of data. Per \citet{bergstra2012random}, optimizing $\HyperParameters$ is achieved by minimizing the generalization error $\mathbb{E}_{X \sim M}[f(\Parameters;\HyperParameters;X)]$ where $X$ is a random variable that represents random data samples and $M$ is some natural distribution. The process of determining optimal values for $\HyperParameters$ is called \textbf{hyper-parameter optimization}, which involves the following:
% \begin{equation}
%     \HyperParameters^* \leftarrow \argmin\limits_{\HyperParameters \in \Lambda}\mathbb{E}_{X \sim M}[f(\Parameters;\HyperParameters;X)] \label{eq:hp_optim}
% \end{equation}
% Unfortunately, neither efficient algorithms exist for solving \eqref{eq:hp_optim} nor can the expectation over $M$ in \eqref{eq:hp_optim} be evaluated \citep{bergstra2012random}. Given this, the process of optimizing the hyper-parameters $\HyperParameters$ in practice is simplified to solving
% \begin{equation}
%     \HyperParameters^* \leftarrow \argmin\limits_{\HyperParameters \in \Lambda}\tau(\HyperParameters) \label{eq:hp_optim_simple}
% \end{equation}
% where $\tau$ is called the \textbf{hyper-parameter response function}, sometimes also called the \textbf{response surface}, and $\Lambda$ is some set of choices for $\HyperParameters$ (\textit{i.e.} the search space). Naturally, different data sets, network architectures, tasks, and learning algorithms will result in different $\tau$ and $\Lambda$. Even given this simplification, generally speaking, very little is known about the nature of $\tau$ and $\Lambda$, and the \textit{de facto} technique for discovering $\HyperParameters^*$ is to define some set $\Lambda \leftarrow \{\HyperParameters^{(1)}, \hdots, \HyperParameters^{(H)}\}$, evaluate $\tau(\HyperParameters^{(i)});\ i \in [H]$, and simply return the best one \citep{bergstra2012random}.

% The dominant techniques for defining $\Lambda$ are manual search, grid search, and random search. Manual search simply involves the use of iterative manual tuning of each $\HyperParameters_i$, $i \in [1, \hdots, K]$ following training experiments until a satisfactory level of performance is achieved. It suffers greatly from irreproducible results and high time consumption. Grid search works by selecting a $g$ values (the number of grid spaces) for each hyper-parameter $\HyperParameters_i$. We now define our set $\boldsymbol{\Lambda} \in \mathbb{R}^{g\times K}$, $|\boldsymbol{\Lambda}_i| = g$, where $\boldsymbol{\lambda}_i;\ i \in [g]$ is the range of values for hyper-parameter $\HyperParameters_i$. Every possible combination of values is made and tested, resulting in $\prod_{k=1}^K |\boldsymbol{\Lambda}_i|$ number of trials, making grid search a very expensive process. Random search operates similarly to grid search, only instead of trialing every possible combination of $\boldsymbol{\Lambda}_i; i \in [1,\hdots,K]$, a random combination is made. Random search improves over grid searching techniques in achieving equivalent or better performance in less computational time \citep{bergstra2012random}. 

% When we restrict our focus to one hyper-parameter in particular, we can simply consider grid searching as the currently regarded optimal technique for discovering the optimal value of that parameter. In particular, we wish only to consider optimization of the initial learning rate for various optimizers (\textit{e.g.} AdaM, AdaGrad, SGD, etc.). Despite a dimensionality reduction in our hyper-parameter set $\HyperParameters$ from $K$ to $1$, grid searching still requires extensive trials of training, which can take numerous days to complete. Even the, it does not provide a guarantee that the final initial learning rate is in fact optimal. Even more, the search space $\Lambda$ is manually defined and quite often undergoes iterations itself, adding time to the process. 

% This expensive, manual process arises from an undefined response surface. In the following, we introduce a tractable response surface that can be used to optimize not only the global learning rate $\GlobalLR$, but any set of hyper-parameters $\HyperParameters \in \mathbb{R}^K$. We will show how our technique, \AlgName, using our response surface, can autonomously set the initial learning rate, without the need for manual intervention in the form of the hyper-parameter set $\Lambda$.
